Why Does My Transaction Fail? A First Look at Failed Transactions on the Solana Blockchain

Solana is an emerging blockchain platform, recognized for its high throughput and low transaction costs, positioning it as a preferred infrastructure for Decentralized Finance (DeFi), Non-Fungible Tokens (NFTs), and other Web 3.0 applications. In the Solana ecosystem, transaction initiators submit various instructions to interact with a diverse range of Solana smart contracts, among which are decentralized exchanges (DEXs) that utilize automated market makers (AMMs), allowing users to trade cryptocurrencies directly on the blockchain without the need for intermediaries. Despite the high throughput and low transaction costs of Solana, the advantages have exposed Solana to bot spamming for financial exploitation, resulting in the prevalence of failed transactions and network congestion. Prior work on Solana has mainly focused on the evaluation of the performance of the Solana blockchain, particularly scalability and transaction throughput, as well as on the improvement of smart contract security, leaving a gap in understanding the characteristics and implications of failed transactions on Solana. To address this gap, we conducted a large-scale empirical study of failed transactions on Solana, using a curated dataset of over 1.5 billion failed transactions across more than 72 million blocks. Specifically, we first characterized the failed transactions in terms of their initiators, failure-triggering programs, and temporal patterns, and compared their block positions and transaction costs with those of successful transactions. We then categorized the failed transactions by the error messages in their error logs, and investigated how specific programs and transaction initiators are associated with these errors...

==> tables/4_RQ2_error.tex <==
\begin{table*}[t]
\centering
  \caption{Error Types in Failed Transactions on Solana.}
  \label{tab:erro_log}
    \begin{tabular}{ccccc}
        \toprule
        \textbf{Error Types} & 
        \textbf{Error Log Example} & 
        \textbf{Count | Percentage}  &\textbf{} \\
        \midrule
        
        \multirow{3}{*}{Price or Profit not met}
        & Slippage tolerance exceeded & \multirow{3}{*}{351,522,390 | 43.88\%} \\
        & IOC order failed to meet minimum fill requirements &   \\
        & No Profit at the end\\
        \midrule
        
        \multirow{3}{*}{Invalid Status}        
        & The amm account owner is not match with this program & \multirow{3}{*}{341,586,093 | 42.64\%} \\
        & Account is frozen &   \\
        & Pyth oracle status is not trading\\
        \midrule
       
        \multirow{3}{*}{Out of Funds}        
        & insufficient funds & \multirow{3}{*}{31,737,032 | 3.96\%} \\
        & Insufficient collateral &   \\
        & insufficient funds for instruction\\
        \midrule

        \multirow{3}{*}{Invalid Input Parameters}        
        & InvalidInput & \multirow{3}{*}{27,496,008 | 3.43\%} \\
        & invalid account data for instruction &   \\
        & invalid program argument\\
        \midrule

        \multirow{3}{*}{Network Delay}        
        & Delay transaction & \multirow{3}{*}{21,617,568 | 2.70\%} \\
        & \small Slot expired &   \\
        & Stale report\\
        \midrule
        
        \multirow{3}{*}{Invalid Input Account}        
        & InvalidSplTokenProgram & \multirow{3}{*}{6,760,053 | 0.84\%} \\
        & Not enough account keys given to the instruction &   \\
        & The given account is not owned by the system program\\
        \midrule

        \multirow{3}{*}{Out of Resource}        
        & memory allocation failed, out of memory & \multirow{3}{*}{4,446,004 | 0.56\%} \\
        & \small exceeded CUs meter at BPF instruction &   \\
        & Computational budget exceeded\\
        \midrule

        \multirow{3}{*}{Program Runtime Error}        
        & panicked at range end index 72 out of range for slice of length 0 & \multirow{3}{*}{352,908 | 0.04\%} \\
        & panicked at called Option::unwrap() on a None value &   \\
        & panicked at attempt to multiply with overflow\\
        \midrule
        
        \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Program Logic \\Constraint Violation\end{tabular}}        
        & Player has not requested a result & \multirow{3}{*}{427,387 | 0.05\%} \\
        & \small A seeds constraint was violated &   \\
        & A raw constraint was violated\\
        \midrule
        
        

        \multirow{3}{*}{Unknown}        
        & 0xdeadbeef & \multirow{3}{*}{13,751,672 | 1.72\%} \\
        & Custom program error: 0x2 &   \\
        & Log truncated\\
        \midrule
        
         \multirow{1}{*}{Uncategorized}
        & - &  1,451,365 | 0.18\% \\
      \bottomrule
    \end{tabular}
\end{table*}
